Reward Learning from Multiple Feedback Types

Learning rewards from preference feedback has become an important tool in the alignment of agentic models. Preference-based feedback, often implemented as a binary comparison between multiple completions, is an established method to acquire large-scale human feedback. However, human feedback in other contexts is often much more diverse. Such diverse feedback can better support the goals of a human annotator, and the simultaneous use of multiple sources might be mutually informative for the learning process or carry type-dependent biases for the reward learning process. Despite these potential benefits, learning from different feedback types has yet to be explored extensively. In this paper, we bridge this gap by enabling experimentation and evaluating multi-type feedback in a broad set of environments. We present a process to generate high-quality simulated feedback of six different types. Then, we implement reward models and downstream RL training for all six feedback types. Based on the simulated feedback, we investigate the use of types of feedback across ten RL environments and compare them to pure preference-based baselines. We show empirically that diverse types of feedback can be utilized and lead to strong reward modeling performance. This work is the first strong indicator of the potential of multi-type feedback for RLHF.

==> algo_backup.tex <==
%% Evaluative
\begin{algorithm}
    \caption{Synthetic Feedback Generation}
    \label{alg:synthetic_feedback_generation}

    \begin{algorithmic}[1]
        \State import gymnasium
        \State
        \State environment = gymnasium.make(environment\_name)
        \State experts = [model.load(expert\_model\_path) for expert\_model\_path in expert\_model\_paths]
        \State
        \State segments = []
        \State
        \For{checkpoint in novice\_model\_checkpoints}
            \State novice = checkpoint.load()
            \State state = environment.reset()
            \State
            \State feedback = []
            \State state\_copies = []
            \State
            \State \# Collect states, actions and rewards from the novice agent
            \For {i in range(steps\_per\_checkpoint)}
                \State state\_copies.append(environment.get\_state())
                \State
                \State novice\_action = novice.predict(state)
                \State next\_novice\_state, novice\_reward = environment.step(novice\_action)
                \State
                \State feedback.append((state, novice\_action, novice\_reward))
            \EndFor
            \State
            \State \# Create segments from individual steps
            \State segments.extend(create\_segments(feedback, segment\_length))
            \State
            \State \# Calculate optimality gaps
            \State optimality\_gaps = []
            \State
            \For {segment in segments}
                \State initial\_value = mean([expert\_value(expert, segment[0]) for expert in experts])
                \State final\_value = mean([expert\_value(expert, segment[-1]) for expert in experts])
                \State
                \State discounted\_reward\_sum = calculate\_discounted\_sum(segment)
                \State
                \State optimal\_reward\_sum = initial\_value - gamma ** len(segment) * final\_value
                \State optimality\_gaps.append(optimal\_reward\_sum - discounted\_reward\_sum)
            \EndFor
            \State
            \State \# Collect evaluative feedback by binning the optimality gaps
            \State evaluative\_feedback = 10 - bin\_indices(optimality\_gaps, 10)
            \State
            \State \# Collect comparative feedback by choosing preference pairs according to optimality gaps
            \State comparative\_feedback = get\_preference\_pairs(segments, optimality\_gaps)
        \EndFor
    \end{algorithmic}
\end{algorithm}

%% Demonstrative
\begin{algorithm}
    \caption{Synthetic Feedback Generation (demonstrative and corrective)}
    \label{alg:synthetic_feedback_generation_demonstrative_corrective}

    \begin{algorithmic}[1]
        \State demonstrative\_feedback = []
        \State corrective\_feedback = []
        \State
        \For {state\_index in len(state\_copies)}
            \State current\_demonstrations = []
            \State current\_expert\_returns = []
            \State
            \State \# Generate demonstrations with all experts, then save the best one
            \For {model\_index in len(expert\_models)}
                \State state = environment.set\_state(state\_copies[state\_index])
                \State
                \State demonstration = []
                \State
                \For {len(segment\_index)}
                    \State expert\_action = expert.predict(state)
                    \State next\_expert\_state, expert\_reward = environment.step(expert\_action)
                    \State
                    \State demonstration.append((state, expert\_action, expert\_reward))
                    \State state = next\_expert\_state
                \EndFor
                \State
                \State current\_demonstrations.append(demonstration)
                \State current\_expert\_returns.append(calculate\_discounted\_sum(demonstration))
            \EndFor
            \State
            \State best\_demonstration\_index = argmax(current\_expert\_returns)
            \State best\_demonstration = current\_demonstrations[best\_demonstration\_index]
            \State best\_demonstration\_return = current\_expert\_returns[best\_demonstration\_index]
            \State original\_return = calculate\_discounted\_sum(segments[state\_index])
            \State
            \If {best\_demonstration\_return \textless original\_return}
                \State demonstrative\_feedback.append(best\_demonstration)
                \State corrective\_feedback.append((segments[state\_index], best\_demonstration))
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}

%% Descriptive
\begin{algorithm}
    \caption{Synthetic Feedback Generation (descriptive)}
    \label{alg:synthetic_feedback_generation_descriptive}

    \begin{algorithmic}[1]
        \State states = []
        \State rewards = []
        \State
        \For {segment in segments}
            \State states.append(concatenate([(step["state"], step["action"]) for step in segment]))
            \State rewards.append(concatenate([step["reward"] for step in segment]))
        \EndFor
        \State
        \State states = concatenate(states)
        \State rewards = concatenate(rewards)
        \State
        \State \# Cluster observations and actions, then calculate a representative for each cluster
        \State cluster\_assignments = cluster\_with\_kmeans(states, len(feedback))
        \State
        \State cluster\_representatives = [mean(states[cluster\_mask]) for cluster\_mask in cluster\_assignments]
        \State cluster\_rewards = [mean(rewards[cluster\_mask]) for cluster\_mask in cluster\_assignments]
        \State
        \State descriptive\_preferences = get\_preference\_pairs(cluster\_representatives, cluster\_rewards)
    \end{algorithmic}
\end{algorithm}
